LRTuner: A Learning Rate Tuner for Deep Neural Networks

One very important hyperparameter for training deep neural networks is the learning rate schedule of the optimizer. The choice of learning rate schedule determines the computational cost of getting close to a minima, how close you actually get to the minima, and most importantly the kind of local minima (wide/narrow) attained. The kind of minima attained has a significant impact on the generalization accuracy of the network. Current systems employ hand tuned learning rate schedules, which are painstakingly tuned for each network and dataset. Given that the state space of schedules is huge, finding a satisfactory learning rate schedule can be very time consuming. In this paper, we present LRTuner, a method for tuning the learning rate as training proceeds. Our method works with any optimizer, and we demonstrate results on SGD with Momentum, and Adam optimizers. We extensively evaluate LRTuner on multiple datasets, models, and across optimizers. We compare favorably against standard learning rate schedules for the given dataset and models, including ImageNet on Resnet-50, Cifar-10 on Resnet-18, and SQuAD fine-tuning on BERT. For example on ImageNet with Resnet-50, LRTuner shows up to 0.2% absolute gains in test accuracy compared to the hand-tuned baseline schedule. Moreover, LRTuner can achieve the same accuracy as the baseline schedule in 29% less optimization steps.

==> sections/algorithm.tex <==
	% Insert the algorithm
	\begin{algorithm}
		\caption{Optimizer Step}
		\label{alg:optimizer_step}
		\begin{algorithmic}[1]
		  %  \Input{hhh}
			\Procedure{Step}{$\Theta$, $loss$}
			
			\If{recalculation_window_crossed()}
			    computeBestLR()
			\Else
			    DoNothing
			\Endif
			
			\State $G = \{X , E_{pos} , E_{neg} \}$ %\Comment{ Eq. and Eq. }
			\For { $k^\prime \in \{1, 2, \dots, k \}$ }
			\State $ x_{max} =  \argmax_{x \in \textbf{X}} \{|(x , x^\prime) \in E_{pos}|\} $
			\State $S_{k^\prime} = \{x : (x,x_{max}) \in E_{pos}\} \cup \{x_{max}\} $
			
    			\For { $x^\prime \in \textbf{X}$ }
    			    \State Remove $x^\prime$ from $G$, if $(x^\prime,x_{max}) \notin E_{neg}$
    			\EndFor
			\EndFor
			\State Return $\textbf{S} = \{S_1, S_2, \dots, S_k\}$
			\EndProcedure
		\end{algorithmic}
	\end{algorithm}

==> sections/extra_baselines.tex <==
\section{Comparisons with More Baseline Learning Rate Schedules}
\label{sec:extra_baselines}

In this section we compare \system{} against more learning rate schedules -- one-cycle, linear decay and cosine decay.

\textbf{One-Cycle}: The one-cycle learning rate schedule was proposed in \cite{smith2018disciplined_onecycle} (also see \cite{smith2017cyclical}). This schedule first chooses a maximum learning rate based on an LR Range test. The LR range test starts from a small learning rate and keeps increasing the learning rate until the loss starts exploding. \cite{smith2018disciplined_onecycle} suggests that the maximum learning rate should be chosen to be bit before the minima, in a region where the loss is still decreasing. There is subjectivity in making this choice, although some blogs and libraries\footnote{See e.g. \url{https://towardsdatascience.com/finding-good-learning-rate-and-the-one-cycle-policy-7159fe1db5d6} and \url{https://sgugger.github.io/how-do-you-find-a-good-learning-rate.html}. Also see \url{https://docs.fast.ai/callbacks.lr_finder.html} and \url{https://docs.fast.ai/callbacks.one_cycle.html}} suggest using a learning rate one order lower than the one at minima. However, in our experience, we found that this choice did not perform well. Instead, we found that values closer to the minima performed much better. In the experiments below we tried multiple values closer to the minima where the loss was still decreasing and report the best results as \textit{one-cycle (tuned)}. Results with the default policy of $1/10^{th}$ the minima are reported as \textit{one-cycle (default)}.

Once the maximum learning rate is chosen, the one-cycle schedule proceeds as follows. The learning rate starts at a specified fraction\footnote{See div\_factor in \url{https://docs.fast.ai/callbacks.one_cycle.html}. We chose the fraction to be 0.1 in our experiments.} of the maximum learning rate and is increased linearly to the maximum learning rate for 45 percent of the training budget and then decreased linearly for the remaining 45. For the final 10 percent, the learning rate is reduced by a large factor (we chose a factor of 10). For the Momentum optimizer, \cite{smith2018disciplined_onecycle} suggests to reduce the momentum linearly when lr is increasing, and vice versa. We used an opensource implementation \footnote{\url{https://github.com/nachiket273/One_Cycle_Policy} } for our experiments.

\textbf{Trapezoid}: The trapezoid learning rate schedule was proposed in \cite{walk-with-sgd-2018}, and is a variation on the one-cycle schedule. The trapezoid schedule increases the learning rate as in the first phase of one-cycle, but then keeps it flat at that value for sometime, before linearly decaying it again like the second phase of one-cycle. Following the Trapezoid (long) schedule of \cite{walk-with-sgd-2018} (see Figure 7,8 there), in all our experiments we linearly warmup for the first $10\%$ of iterations, stay flat for the next $80\%$, and then linearly decay for the final $10\%$ iterations. For the maximum learning rate we use the values of the tuned one-cycle runs.


\textbf{Linear Decay}: The linear decay learning rate schedule simply decays the learning rate linearly to zero starting from a seed LR. In the case of IWSLT we found that starting from a high seed caused instability issues (most likely because of Adam optimizer. See \cite{liu2019variance_radam}). In this case we also ran experiments with a linear warmup followed by this linear decay.

\textbf{Cosine Decay}: The cosine decay learning rate schedule decays the learning rate to zero following a cosine curve, starting from a seed LR. Similar to Linear decay, in the case of IWSLT, we found that starting from a high seed caused instability issues. In this case we also ran experiments with a linear warmup followed by this cosine decay.

\begin{figure}[h]
    \begin{subfigure}[t]{0.32\textwidth}
        \centering
        \includegraphics[width=0.99\linewidth]{figures/one_cycle/lr_cifar.pdf}
        \caption{LR Range test for CIFAR-10}
        \label{fig:lr_range_test_cifar}
    \end{subfigure}
    \begin{subfigure}[t]{0.32\textwidth}
        \centering
        \includegraphics[width=0.99\linewidth]{figures/one_cycle/lr_fairseq.pdf}
        \caption{LR Range test for IWSLT}
        \label{fig:lr_range_test_iwslt}
    \end{subfigure}
    \begin{subfigure}[t]{0.32\textwidth}
        \centering
        \includegraphics[width=0.99\linewidth]{figures/one_cycle/lr_bert.pdf}
        \caption{LR Range test for SQuAD}
        \label{fig:lr_range_test_bert_squad}
    \end{subfigure}
\caption{LR Range test for selecting the maximum learning rate. A good choice is the learning rate is a bit before the minima in a region where the loss is still decreasing.}
\label{fig:lr_range_tests}
\end{figure}

\subsection{Cifar-10}
Figure~\ref{fig:lr_range_test_cifar} shows the LR range test for Cifar-10 with the Resnet-18 network. The minima occurs around learning rate of 0.09. For the maximum learning rate, we choose 9e-3 for the default one-cycle policy, but found 0.06 to perform best in our tuning. For linear, cosine decay schedules we start with a seed learning rate of 0.1 as used in the standard baselines. Table~\ref{tab:cifar_results_extra_baselines} shows the training loss and test accuracy for the various schedules.

\begin{table}[h]
\small
\centering
{\setlength{\extrarowheight}{1pt}%
\begin{tabular}{|c|c|c|}
  \hline
  LR Schedule      & Train Loss & Test Accuracy \\ \hline
  Trapezoid           & 0.0009 (8.7e-5) & 94.69 (0.0007)    \\
  One-Cycle (default) & 0.0003 (3e-5)   & 93.38 (0.001) \\
  One-Cycle (tuned)   & 0.0004 (3.1e-5) & 94.59 (0.0007) \\
  Cosine Decay        & 0.0003 (2.7e-5) & 94.52 (0.0016) \\
  Linear Decay        & 0.0002 (2.5e-5) & 94.24 (0.0009) \\
  \system{}           & 0.0008 (1.0e-4) & 94.79 (0.001) \\ \hline
\end{tabular}}
\caption{Training loss and Test accuracy for Cifar-10 on Resnet-18 for more learning rate schedules. We report the mean and standard deviation over 7 runs. For One-Cycle, we report experiments with maximum learning rate chosen via the default lr-range finder policy and via manual tuning. The Trapezoid schedule uses maximum learning rate of the tuned setting.}
\label{tab:cifar_results_extra_baselines}
\end{table}


\subsection{IWSLT'14 DE-EN}
Figure~\ref{fig:lr_range_test_iwslt} shows the LR range test for IWSLT on the transformer networks. The minima occurs at 9e-4. For the maximum learning rate, we choose 9e-5 for the default one-cycle policy and found 2e-4 to perform best in our tuning. For linear, cosine decay schedules we first used a seed learning rate of 5e-4 (the maximum learning rate in the schedule in \cite{vaswani2017attention}). However, we found this to perform very poorly, most likely due to initial instabilities in Adam as discussed in \cite{liu2019variance_radam}. So we also ran experiments with linear warmup as in \cite{vaswani2017attention} followed by linear/cosine decays which performed much better. Table~\ref{tab:iwslt_results_extra_baselines} shows the training, validation perplexity and BLEU scores for the various schedules.

\begin{table}[h]
\small
\centering
{\setlength{\extrarowheight}{1pt}%
\begin{tabular}{|c|c|c|c|}
  \hline
  LR Schedule & Train ppl & Validation ppl & Test BLEU Score   \\ \hline
  Trapezoid           & 3.25 (0.016)           & 4.92 (0.014)          & 34.85 (0.008)          \\
  One-Cycle (default) & 5.51 (0.028) & 5.87 (0.02) &  32.35 (0.18) \\
  One-Cycle (tuned)   & 3.82 (0.09) & 5.01 (0.03) & 34.57 (0.002) \\
  Cosine Decay & 9.54 (0.06) & 3861.6 (883.4) &  0.33 (1e-5)\\
  Cosine Decay with warmup  & 3.29 (0.02) & 5.04 (0.019) & 34.85 (0.008) \\
  Linear Decay & 9.50 (0.07) & 3261.5 (849.7) &  0.28 (2e-5)\\
  Linear Decay with warmup  & 3.30(0.02) & 5.03 (0.016) & 34.82 (0.006) \\                     
  \system{} & 3.46 (0.16)  & 4.86 (0.014) & 34.88 (0.005) \\ \hline
\end{tabular}}
\caption{Training, validation perplexity and test BLEU scores for IWSLT on Transformer networks for more learning rate schedules.
The test BLEU scores are computed on the checkpoint with the best validation perplexity. We report
the mean and standard deviation over 3 runs.}
\label{tab:iwslt_results_extra_baselines}
\end{table}

\subsection{SQuAD-v1.1}
Figure~\ref{fig:lr_range_test_bert_squad} show the LR range test for SQuAD fine-tuning on BERT. The minima occurs at 1e-4. For the maximum learning rate, we choose 1e-5 for the default one-cycle policy and found 4e-5 to perform best in our tuning. For linear, cosine decays we start with a seed learning rate of 2e-5 as used in \cite{devlin2018bert}. Table~\ref{tab:squad_results_extra_baselines} show the average training loss, best test EM score, and
average test EM, F1 scores for the various schedules.

\begin{table}[h]
\small
\centering
{\setlength{\extrarowheight}{1pt}%
\begin{tabular}{|c|c|c|c|c|}
  \hline
  LR Schedule          & Train Loss (av) & EM (best) & EM (av)  & F1 (av) \\ \hline
  Trapezoid            &    0.95(0.002)  & 80.2   & 80.1 (0.05) & 87.9 (0.04) \\
  One Cycle (default)  & 1.364 (0.011)   & 79.8   & 79.4 (0.17) & 87.3 (0.12) \\
  One Cycle (tuned)    & 1.016 (0.004)   & 80.9   & 80.7 (0.12) & 88.4 (0.09) \\
  Cosine Decay         & 0.89 (0.003)    & 80.8   & 80.6 (0.06) & 88.4 (0.13) \\
  Linear decay         & 0.96 (0.075)    & 80.7   & 80.4 (0.18) & 88.2 (0.02) \\
  \system{}            & 1.05 (0.008)    & 81.2   & 80.8 (0.52) & 88.5 (0.09) \\ \hline
\end{tabular}}
\caption{SQuAD fine-tuning on BERT for more learning rate schedules. We report the average training loss, best test EM score, and
average test EM, F1 scores over 3 runs.}
\label{tab:squad_results_extra_baselines}
\end{table}

==> sections/math_commands.tex <==
%%%%% NEW MATH DEFINITIONS %%%%%

\usepackage{amsmath,amsfonts,bm}

% Mark sections of captions for referring to divisions of figures
\newcommand{\figleft}{{\em (Left)}}
\newcommand{\figcenter}{{\em (Center)}}
\newcommand{\figright}{{\em (Right)}}
\newcommand{\figtop}{{\em (Top)}}
\newcommand{\figbottom}{{\em (Bottom)}}
\newcommand{\captiona}{{\em (a)}}
\newcommand{\captionb}{{\em (b)}}
\newcommand{\captionc}{{\em (c)}}
\newcommand{\captiond}{{\em (d)}}

% Highlight a newly defined term
\newcommand{\newterm}[1]{{\bf #1}}


% Figure reference, lower-case.
\def\figref#1{figure~\ref{#1}}
% Figure reference, capital. For start of sentence
\def\Figref#1{Figure~\ref{#1}}
\def\twofigref#1#2{figures \ref{#1} and \ref{#2}}
\def\quadfigref#1#2#3#4{figures \ref{#1}, \ref{#2}, \ref{#3} and \ref{#4}}
% Section reference, lower-case.
\def\secref#1{section~\ref{#1}}
% Section reference, capital.
\def\Secref#1{Section~\ref{#1}}
% Reference to two sections.
\def\twosecrefs#1#2{sections \ref{#1} and \ref{#2}}
% Reference to three sections.
\def\secrefs#1#2#3{sections \ref{#1}, \ref{#2} and \ref{#3}}
% Reference to an equation, lower-case.
\def\eqref#1{equation~\ref{#1}}
% Reference to an equation, upper case
\def\Eqref#1{Equation~\ref{#1}}
% A raw reference to an equation---avoid using if possible
\def\plaineqref#1{\ref{#1}}
% Reference to a chapter, lower-case.
\def\chapref#1{chapter~\ref{#1}}
% Reference to an equation, upper case.
\def\Chapref#1{Chapter~\ref{#1}}
% Reference to a range of chapters
\def\rangechapref#1#2{chapters\ref{#1}--\ref{#2}}
% Reference to an algorithm, lower-case.
\def\algref#1{algorithm~\ref{#1}}
% Reference to an algorithm, upper case.
\def\Algref#1{Algorithm~\ref{#1}}
\def\twoalgref#1#2{algorithms \ref{#1} and \ref{#2}}
\def\Twoalgref#1#2{Algorithms \ref{#1} and \ref{#2}}
% Reference to a part, lower case
\def\partref#1{part~\ref{#1}}
% Reference to a part, upper case
\def\Partref#1{Part~\ref{#1}}
\def\twopartref#1#2{parts \ref{#1} and \ref{#2}}

\def\ceil#1{\lceil #1 \rceil}
\def\floor#1{\lfloor #1 \rfloor}
\def\1{\bm{1}}
\newcommand{\train}{\mathcal{D}}
\newcommand{\valid}{\mathcal{D_{\mathrm{valid}}}}
\newcommand{\test}{\mathcal{D_{\mathrm{test}}}}

\def\eps{{\epsilon}}


% Random variables
\def\reta{{\textnormal{$\eta$}}}
\def\ra{{\textnormal{a}}}
\def\rb{{\textnormal{b}}}
\def\rc{{\textnormal{c}}}
\def\rd{{\textnormal{d}}}
\def\re{{\textnormal{e}}}
\def\rf{{\textnormal{f}}}
\def\rg{{\textnormal{g}}}
\def\rh{{\textnormal{h}}}
\def\ri{{\textnormal{i}}}
\def\rj{{\textnormal{j}}}
\def\rk{{\textnormal{k}}}
\def\rl{{\textnormal{l}}}
% rm is already a command, just don't name any random variables m
\def\rn{{\textnormal{n}}}
\def\ro{{\textnormal{o}}}
\def\rp{{\textnormal{p}}}
\def\rq{{\textnormal{q}}}
\def\rr{{\textnormal{r}}}
\def\rs{{\textnormal{s}}}
\def\rt{{\textnormal{t}}}
\def\ru{{\textnormal{u}}}
\def\rv{{\textnormal{v}}}
\def\rw{{\textnormal{w}}}
\def\rx{{\textnormal{x}}}
\def\ry{{\textnormal{y}}}
\def\rz{{\textnormal{z}}}

% Random vectors
\def\rvepsilon{{\mathbf{\epsilon}}}
\def\rvtheta{{\mathbf{\theta}}}
\def\rva{{\mathbf{a}}}
\def\rvb{{\mathbf{b}}}
\def\rvc{{\mathbf{c}}}
\def\rvd{{\mathbf{d}}}
\def\rve{{\mathbf{e}}}
\def\rvf{{\mathbf{f}}}
\def\rvg{{\mathbf{g}}}
\def\rvh{{\mathbf{h}}}
\def\rvu{{\mathbf{i}}}
\def\rvj{{\mathbf{j}}}
\def\rvk{{\mathbf{k}}}
\def\rvl{{\mathbf{l}}}
\def\rvm{{\mathbf{m}}}
\def\rvn{{\mathbf{n}}}
\def\rvo{{\mathbf{o}}}
\def\rvp{{\mathbf{p}}}
\def\rvq{{\mathbf{q}}}
\def\rvr{{\mathbf{r}}}
\def\rvs{{\mathbf{s}}}
\def\rvt{{\mathbf{t}}}
\def\rvu{{\mathbf{u}}}
\def\rvv{{\mathbf{v}}}
\def\rvw{{\mathbf{w}}}
\def\rvx{{\mathbf{x}}}
\def\rvy{{\mathbf{y}}}
\def\rvz{{\mathbf{z}}}

% Elements of random vectors
\def\erva{{\textnormal{a}}}
\def\ervb{{\textnormal{b}}}
\def\ervc{{\textnormal{c}}}
\def\ervd{{\textnormal{d}}}
\def\erve{{\textnormal{e}}}
\def\ervf{{\textnormal{f}}}
\def\ervg{{\textnormal{g}}}
\def\ervh{{\textnormal{h}}}
\def\ervi{{\textnormal{i}}}
\def\ervj{{\textnormal{j}}}
\def\ervk{{\textnormal{k}}}
\def\ervl{{\textnormal{l}}}
\def\ervm{{\textnormal{m}}}
\def\ervn{{\textnormal{n}}}
\def\ervo{{\textnormal{o}}}
\def\ervp{{\textnormal{p}}}
\def\ervq{{\textnormal{q}}}
\def\ervr{{\textnormal{r}}}
\def\ervs{{\textnormal{s}}}
\def\ervt{{\textnormal{t}}}
\def\ervu{{\textnormal{u}}}
\def\ervv{{\textnormal{v}}}
\def\ervw{{\textnormal{w}}}
\def\ervx{{\textnormal{x}}}
\def\ervy{{\textnormal{y}}}
\def\ervz{{\textnormal{z}}}

% Random matrices
\def\rmA{{\mathbf{A}}}
\def\rmB{{\mathbf{B}}}
\def\rmC{{\mathbf{C}}}
\def\rmD{{\mathbf{D}}}
\def\rmE{{\mathbf{E}}}
\def\rmF{{\mathbf{F}}}
\def\rmG{{\mathbf{G}}}
\def\rmH{{\mathbf{H}}}
\def\rmI{{\mathbf{I}}}
\def\rmJ{{\mathbf{J}}}
\def\rmK{{\mathbf{K}}}
\def\rmL{{\mathbf{L}}}
\def\rmM{{\mathbf{M}}}
\def\rmN{{\mathbf{N}}}
\def\rmO{{\mathbf{O}}}
\def\rmP{{\mathbf{P}}}
\def\rmQ{{\mathbf{Q}}}
\def\rmR{{\mathbf{R}}}
\def\rmS{{\mathbf{S}}}
\def\rmT{{\mathbf{T}}}
\def\rmU{{\mathbf{U}}}
\def\rmV{{\mathbf{V}}}
\def\rmW{{\mathbf{W}}}
\def\rmX{{\mathbf{X}}}
\def\rmY{{\mathbf{Y}}}
\def\rmZ{{\mathbf{Z}}}

% Elements of random matrices
\def\ermA{{\textnormal{A}}}
\def\ermB{{\textnormal{B}}}
\def\ermC{{\textnormal{C}}}
\def\ermD{{\textnormal{D}}}
\def\ermE{{\textnormal{E}}}
\def\ermF{{\textnormal{F}}}
\def\ermG{{\textnormal{G}}}
\def\ermH{{\textnormal{H}}}
\def\ermI{{\textnormal{I}}}
\def\ermJ{{\textnormal{J}}}
\def\ermK{{\textnormal{K}}}
\def\ermL{{\textnormal{L}}}
\def\ermM{{\textnormal{M}}}
\def\ermN{{\textnormal{N}}}
\def\ermO{{\textnormal{O}}}
\def\ermP{{\textnormal{P}}}
\def\ermQ{{\textnormal{Q}}}
\def\ermR{{\textnormal{R}}}
\def\ermS{{\textnormal{S}}}
\def\ermT{{\textnormal{T}}}
\def\ermU{{\textnormal{U}}}
\def\ermV{{\textnormal{V}}}
\def\ermW{{\textnormal{W}}}
\def\ermX{{\textnormal{X}}}
\def\ermY{{\textnormal{Y}}}
\def\ermZ{{\textnormal{Z}}}

% Vectors
\def\vzero{{\bm{0}}}
\def\vone{{\bm{1}}}
\def\vmu{{\bm{\mu}}}
\def\vtheta{{\bm{\theta}}}
\def\va{{\bm{a}}}
\def\vb{{\bm{b}}}
\def\vc{{\bm{c}}}
\def\vd{{\bm{d}}}
\def\ve{{\bm{e}}}
\def\vf{{\bm{f}}}
\def\vg{{\bm{g}}}
\def\vh{{\bm{h}}}
\def\vi{{\bm{i}}}
\def\vj{{\bm{j}}}
\def\vk{{\bm{k}}}
\def\vl{{\bm{l}}}
\def\vm{{\bm{m}}}
\def\vn{{\bm{n}}}
\def\vo{{\bm{o}}}
\def\vp{{\bm{p}}}
\def\vq{{\bm{q}}}
\def\vr{{\bm{r}}}
\def\vs{{\bm{s}}}
\def\vt{{\bm{t}}}
\def\vu{{\bm{u}}}
\def\vv{{\bm{v}}}
\def\vw{{\bm{w}}}
\def\vx{{\bm{x}}}
\def\vy{{\bm{y}}}
\def\vz{{\bm{z}}}

% Elements of vectors
\def\evalpha{{\alpha}}
\def\evbeta{{\beta}}
\def\evepsilon{{\epsilon}}
\def\evlambda{{\lambda}}
\def\evomega{{\omega}}
\def\evmu{{\mu}}
\def\evpsi{{\psi}}
\def\evsigma{{\sigma}}
\def\evtheta{{\theta}}
\def\eva{{a}}
\def\evb{{b}}
\def\evc{{c}}
\def\evd{{d}}
\def\eve{{e}}
\def\evf{{f}}
\def\evg{{g}}
\def\evh{{h}}
\def\evi{{i}}
\def\evj{{j}}
\def\evk{{k}}
\def\evl{{l}}
\def\evm{{m}}
\def\evn{{n}}
\def\evo{{o}}
\def\evp{{p}}
\def\evq{{q}}
\def\evr{{r}}
\def\evs{{s}}
\def\evt{{t}}
\def\evu{{u}}
\def\evv{{v}}
\def\evw{{w}}
\def\evx{{x}}
\def\evy{{y}}
\def\evz{{z}}

% Matrix
\def\mA{{\bm{A}}}
\def\mB{{\bm{B}}}
\def\mC{{\bm{C}}}
\def\mD{{\bm{D}}}
\def\mE{{\bm{E}}}
\def\mF{{\bm{F}}}
\def\mG{{\bm{G}}}
\def\mH{{\bm{H}}}
\def\mI{{\bm{I}}}
\def\mJ{{\bm{J}}}
\def\mK{{\bm{K}}}
\def\mL{{\bm{L}}}
\def\mM{{\bm{M}}}
\def\mN{{\bm{N}}}
\def\mO{{\bm{O}}}
\def\mP{{\bm{P}}}
\def\mQ{{\bm{Q}}}
\def\mR{{\bm{R}}}
\def\mS{{\bm{S}}}
\def\mT{{\bm{T}}}
\def\mU{{\bm{U}}}
\def\mV{{\bm{V}}}
\def\mW{{\bm{W}}}
\def\mX{{\bm{X}}}
\def\mY{{\bm{Y}}}
\def\mZ{{\bm{Z}}}
\def\mBeta{{\bm{\beta}}}
\def\mPhi{{\bm{\Phi}}}
\def\mLambda{{\bm{\Lambda}}}
\def\mSigma{{\bm{\Sigma}}}

% Tensor
\DeclareMathAlphabet{\mathsfit}{\encodingdefault}{\sfdefault}{m}{sl}
\SetMathAlphabet{\mathsfit}{bold}{\encodingdefault}{\sfdefault}{bx}{n}
\newcommand{\tens}[1]{\bm{\mathsfit{#1}}}
\def\tA{{\tens{A}}}
\def\tB{{\tens{B}}}
\def\tC{{\tens{C}}}
\def\tD{{\tens{D}}}
\def\tE{{\tens{E}}}
\def\tF{{\tens{F}}}
\def\tG{{\tens{G}}}
\def\tH{{\tens{H}}}
\def\tI{{\tens{I}}}
\def\tJ{{\tens{J}}}
\def\tK{{\tens{K}}}
\def\tL{{\tens{L}}}
\def\tM{{\tens{M}}}
\def\tN{{\tens{N}}}
\def\tO{{\tens{O}}}
\def\tP{{\tens{P}}}
\def\tQ{{\tens{Q}}}
\def\tR{{\tens{R}}}
\def\tS{{\tens{S}}}
\def\tT{{\tens{T}}}
\def\tU{{\tens{U}}}
\def\tV{{\tens{V}}}
\def\tW{{\tens{W}}}
\def\tX{{\tens{X}}}
\def\tY{{\tens{Y}}}
\def\tZ{{\tens{Z}}}


% Graph
\def\gA{{\mathcal{A}}}
\def\gB{{\mathcal{B}}}
\def\gC{{\mathcal{C}}}
\def\gD{{\mathcal{D}}}
\def\gE{{\mathcal{E}}}
\def\gF{{\mathcal{F}}}
\def\gG{{\mathcal{G}}}
\def\gH{{\mathcal{H}}}
\def\gI{{\mathcal{I}}}
\def\gJ{{\mathcal{J}}}
\def\gK{{\mathcal{K}}}
\def\gL{{\mathcal{L}}}
\def\gM{{\mathcal{M}}}
\def\gN{{\mathcal{N}}}
\def\gO{{\mathcal{O}}}
\def\gP{{\mathcal{P}}}
\def\gQ{{\mathcal{Q}}}
\def\gR{{\mathcal{R}}}
\def\gS{{\mathcal{S}}}
\def\gT{{\mathcal{T}}}
\def\gU{{\mathcal{U}}}
\def\gV{{\mathcal{V}}}
\def\gW{{\mathcal{W}}}
\def\gX{{\mathcal{X}}}
\def\gY{{\mathcal{Y}}}
\def\gZ{{\mathcal{Z}}}

% Sets
\def\sA{{\mathbb{A}}}
\def\sB{{\mathbb{B}}}
\def\sC{{\mathbb{C}}}
\def\sD{{\mathbb{D}}}
% Don't use a set called E, because this would be the same as our symbol
% for expectation.
\def\sF{{\mathbb{F}}}
\def\sG{{\mathbb{G}}}
\def\sH{{\mathbb{H}}}
\def\sI{{\mathbb{I}}}
\def\sJ{{\mathbb{J}}}
\def\sK{{\mathbb{K}}}
\def\sL{{\mathbb{L}}}
\def\sM{{\mathbb{M}}}
\def\sN{{\mathbb{N}}}
\def\sO{{\mathbb{O}}}
\def\sP{{\mathbb{P}}}
\def\sQ{{\mathbb{Q}}}
\def\sR{{\mathbb{R}}}
\def\sS{{\mathbb{S}}}
\def\sT{{\mathbb{T}}}
\def\sU{{\mathbb{U}}}
\def\sV{{\mathbb{V}}}
\def\sW{{\mathbb{W}}}
\def\sX{{\mathbb{X}}}
\def\sY{{\mathbb{Y}}}
\def\sZ{{\mathbb{Z}}}

% Entries of a matrix
\def\emLambda{{\Lambda}}
\def\emA{{A}}
\def\emB{{B}}
\def\emC{{C}}
\def\emD{{D}}
\def\emE{{E}}
\def\emF{{F}}
\def\emG{{G}}
\def\emH{{H}}
\def\emI{{I}}
\def\emJ{{J}}
\def\emK{{K}}
\def\emL{{L}}
\def\emM{{M}}
\def\emN{{N}}
\def\emO{{O}}
\def\emP{{P}}
\def\emQ{{Q}}
\def\emR{{R}}
\def\emS{{S}}
\def\emT{{T}}
\def\emU{{U}}
\def\emV{{V}}
\def\emW{{W}}
\def\emX{{X}}
\def\emY{{Y}}
\def\emZ{{Z}}
\def\emSigma{{\Sigma}}

% entries of a tensor
% Same font as tensor, without \bm wrapper
\newcommand{\etens}[1]{\mathsfit{#1}}
\def\etLambda{{\etens{\Lambda}}}
\def\etA{{\etens{A}}}
\def\etB{{\etens{B}}}
\def\etC{{\etens{C}}}
\def\etD{{\etens{D}}}
\def\etE{{\etens{E}}}
\def\etF{{\etens{F}}}
\def\etG{{\etens{G}}}
\def\etH{{\etens{H}}}
\def\etI{{\etens{I}}}
\def\etJ{{\etens{J}}}
\def\etK{{\etens{K}}}
\def\etL{{\etens{L}}}
\def\etM{{\etens{M}}}
\def\etN{{\etens{N}}}
\def\etO{{\etens{O}}}
\def\etP{{\etens{P}}}
\def\etQ{{\etens{Q}}}
\def\etR{{\etens{R}}}
\def\etS{{\etens{S}}}
\def\etT{{\etens{T}}}
\def\etU{{\etens{U}}}
\def\etV{{\etens{V}}}
\def\etW{{\etens{W}}}
\def\etX{{\etens{X}}}
\def\etY{{\etens{Y}}}
\def\etZ{{\etens{Z}}}

% The true underlying data generating distribution
\newcommand{\pdata}{p_{\rm{data}}}
% The empirical distribution defined by the training set
\newcommand{\ptrain}{\hat{p}_{\rm{data}}}
\newcommand{\Ptrain}{\hat{P}_{\rm{data}}}
% The model distribution
\newcommand{\pmodel}{p_{\rm{model}}}
\newcommand{\Pmodel}{P_{\rm{model}}}
\newcommand{\ptildemodel}{\tilde{p}_{\rm{model}}}
% Stochastic autoencoder distributions
\newcommand{\pencode}{p_{\rm{encoder}}}
\newcommand{\pdecode}{p_{\rm{decoder}}}
\newcommand{\precons}{p_{\rm{reconstruct}}}

\newcommand{\laplace}{\mathrm{Laplace}} % Laplace distribution

\newcommand{\E}{\mathbb{E}}
\newcommand{\Ls}{\mathcal{L}}
\newcommand{\R}{\mathbb{R}}
\newcommand{\emp}{\tilde{p}}
\newcommand{\lr}{\alpha}
\newcommand{\reg}{\lambda}
\newcommand{\rect}{\mathrm{rectifier}}
\newcommand{\softmax}{\mathrm{softmax}}
\newcommand{\sigmoid}{\sigma}
\newcommand{\softplus}{\zeta}
\newcommand{\KL}{D_{\mathrm{KL}}}
\newcommand{\Var}{\mathrm{Var}}
\newcommand{\standarderror}{\mathrm{SE}}
\newcommand{\Cov}{\mathrm{Cov}}
% Wolfram Mathworld says $L^2$ is for function spaces and $\ell^2$ is for vectors
% But then they seem to use $L^2$ for vectors throughout the site, and so does
% wikipedia.
\newcommand{\normlzero}{L^0}
\newcommand{\normlone}{L^1}
\newcommand{\normltwo}{L^2}
\newcommand{\normlp}{L^p}
\newcommand{\normmax}{L^\infty}

\newcommand{\parents}{Pa} % See usage in notation.tex. Chosen to match Daphne's book.

\DeclareMathOperator*{\argmax}{arg\,max}
\DeclareMathOperator*{\argmin}{arg\,min}

\DeclareMathOperator{\sign}{sign}
\DeclareMathOperator{\Tr}{Tr}
\let\ab\allowbreak


==> sections/more_results.tex <==
\section{More Results}

\subsection{MNIST}
\label{sec:results_mnist}

In this experiment we trained the MNIST dataset~\cite{mnist_lecun1998gradient} on a 4 layer network with two convolution layers and two fully connected layers \footnote{We used the implementation at: https://github.com/pytorch/examples/tree/master/mnist}. We evaluated our method on SGD, SGD with momentum and Adam optimizers. For baseline runs, we used a fixed learning rate of 0.1 for SGD, Momentum, and 1e-3 for Adam; and trained for 50 epochs. With \system{}, we trained the network with 10 explore epochs, and used the same seed learning rate as baseline, i.e. 0.1 for SGD, Momentum, and 1e-3 for Adam. Table~\ref{tab:mnist_results_train_loss_test_acc} shows the training loss and test accuracy for the various runs. See figures~\ref{fig:mnist_sgd_result}, \ref{fig:mnist_momentum_result}, \ref{fig:mnist_adam_result} for more detailed comparisons of training loss, test accuracy, and learning rate for SGD, Momentum and Adam optimizers, respectively.

\begin{table}[h]
\small
\centering
{\setlength{\extrarowheight}{1pt}%
\begin{tabular}{|c|c|c|c|}
  \hline
  \multirow{2}{*}{LR Schedule} & \multicolumn{3}{c|}{Optimizer} \\
  & SGD & Momentum & Adam \\ \hline \hline
  \multicolumn{4}{|c|}{Training Loss} \\ %\hline
  Baseline & 2.3e-5 (9.4e-7) & 7.2e-6 (4.2e-7) & 4.5e-3 (1.3e-3) \\
  \system{} & 2.4e-5 (5.5e-6) & 7.3e-6 (7.7e-7) & 3.9e-4 (9.5e-4) \\ \hline \hline
  \multicolumn{4}{|c|}{Test Accuracy}\\ %\hline
  Baseline & 99.32 (3.4e-4) & 99.34 (6.0e-4) & 99.21 (1.2e-3) \\
  \system{} & 99.32 (3.7e-4) & 99.38 (5.1e-4) & 99.35 (7.2e-4) \\ \hline
\end{tabular}}
\caption{Training loss and Test accuracy for MNIST. We report the mean and standard deviation over 7 runs.}
\label{tab:mnist_results_train_loss_test_acc}
\end{table}

\subsection{Fashion MNIST}
\label{sec:results_fashion_mnist}

In this experiment we trained the Fashion MNIST dataset~\cite{xiao2017fashion} on the same 4 layer network as for the MNIST dataset. We evaluated our method on SGD, SGD with momentum and Adam optimizers. For baseline runs, we used a fixed learning rate of 0.1 for SGD, Momentum, and 1e-3 for Adam; and trained for 50 epochs. With \system{}, we trained the network with 10 explore epochs, and used the same seed learning rate as baseline, i.e. 0.1 for SGD, Momentum, and 1e-3 for Adam. Table~\ref{tab:fashionmnist_results_train_loss_test_acc} shows the training loss and test accuracy for the various runs. See figures~\ref{fig:fashion_mnist_sgd_result}, \ref{fig:fashion_mnist_momentum_result}, \ref{fig:fashion_mnist_adam_result} for more detailed comparisons of training loss, test accuracy, and learning rate for SGD, Momentum and Adam optimizers, respectively.

\begin{table}[h]
\small
\centering
{\setlength{\extrarowheight}{1pt}%
\begin{tabular}{|c|c|c|c|}
  \hline
  \multirow{2}{*}{LR Schedule} & \multicolumn{3}{c|}{Optimizer} \\
  & SGD & Momentum & Adam \\ \hline \hline
  \multicolumn{4}{|c|}{Training Loss} \\ %\hline
  Baseline  & 0.005 (0.006) & 0.073 (0.007)   & 0.018 (0.003) \\
  \system{} & 0.001 (0.001) & 4.3e-4 (7.2e-4) & 0.002 (0.006) \\ \hline \hline
  \multicolumn{4}{|c|}{Test Accuracy}\\ %\hline
  Baseline  & 91.33 (0.005) & 89.31 (0.003) & 90.56 (0.003) \\
  \system{} & 91.88 (0.001) & 91.66 (0.002) & 91.65 (0.003) \\ \hline
\end{tabular}}
\caption{Training loss and Test accuracy for FashionMNIST. We report the mean and standard deviation over 7 runs.}
\label{tab:fashionmnist_results_train_loss_test_acc}
\end{table}

\clearpage


==> sections/related_work.tex <==
\section{Related Work}
\label{sec:related_work}

\noindent
{\bf Generalization.}
There has been a lot of work recently on understanding the generalization characteristics of DNNs. \cite{kawaguchi2016deep} found that DNNs have many local minima, but all local minima were also the global minima. It has been observed by several authors that wide minima generalize better than narrow minima (\cite{arora2018stronger,hochreiter1997flat,keskar2016large,jastrzkebski2017three,wang2018identifying}) but there have been other work questioning this hypothesis as well~(\cite{dinh2017sharp,golatkar2019time,guiroy2019towards,jastrzebski_iclr_2019,yoshida2017spectral}).

%Doesn't seem that relevant?
%~\cite{step-size-matters-neurips2018} analyze constant learning rate gradient descent for deep linear networks, and show that step size determines the subset of local optima to which the algorithm can converge.


\cite{keskar2016large} found that small batch SGD generalizes better and lands in wider minima than large batch SGD. However, recent work has been able to generalize quite well even with very large batch sizes (\cite{goyal-imagenet-in-an-hour-2017,large-batch-training-openai-2018,large-batch-training-google-2018}), by scaling the learning rate linearly as a function of the batch size.~\cite{jastrzebski_iclr_2019}
analyze how batch size and learning rate influence the curvature of not only the SGD endpoint but also the whole trajectory. They found that small batch or large step SGD have similar characteristics, and yield smaller and earlier peak of spectral norm as well as smaller largest eigenvalue.~\cite{dinh2017sharp} show analytically using model reparameterization that wide minima can be converted to sharp minima without hurting generalization.~\cite{wang2018identifying} analytically show that generalization of a model is related to the Hessian and propose a new metric for the generalization capability of a model that is unaffected by model reparameterization of~\cite{dinh2017sharp}. ~\cite{yoshida2017spectral} argue that regularizing the spectral norm of the weights of the neural network help them generalize better. On the other hand,~\cite{arora2018stronger} derive generalization bounds by showing that networks with low stable rank (high spectral norm) generalize better.~\cite{guiroy2019towards} looks at generalization in gradient-based meta-learning and they show experimentally that generalization and wide minima are not always correlated. Finally,~\cite{golatkar2019time} show that regularization results in higher test accuracy specifically when it is applied during initial phase of training, similar to the importance of \system\'s explore phase during initial phase of training.



\noindent
{\bf Lower density of wide minima.} \cite{wu2018sgd} compares the sharpness of minima obtained by batch gradient descent (GD) with different learning rates for small neural networks on FashionMNIST and Cifar10 datasets. They find that GD with a given learning rate finds the theoretically sharpest feasible minima for that learning rate. Thus, in the presence of several flatter minimas, GD with lower learning rates does not find them, leading the authors to conjecture that density of sharper minima is perhaps larger than density of wider minima.


\noindent
{\bf Adaptive learning.}
Many adaptive learning rate methods have been developed which adapt the learning rate on a per parameter basis, including AdaGrad (\cite{adagrad_duchi2011adaptive}), ADADELTA (\cite{zeiler2012adadelta}), RMSProp (\cite{rmsprop_tieleman2012lecture}), and Adam (\cite{adam_kingma2014adam}). However, most of these methods still require specifying a global learning rate schedule which impacts the performance significantly. Many methods have been proposed to adaptively tune the global learning rate, such as \cite{no_more_pesky_lr_schaul2013} which makes an idealized quadratic loss function assumption near the minima, \cite{baydin2017online_hypergradient} which uses gradient w.r.t the learning rate to update the learning rate in a first order fashion, and \cite{l4-neurips2018} which again uses a first order method along with an estimate of minimum loss achievable in a step. While \cite{no_more_pesky_lr_schaul2013} and \cite{baydin2017online_hypergradient} compare to only constant learning rate baselines, \cite{l4-neurips2018} does compare to state-of-the-art learning rate schedule for Cifar-10, but is unable to match their test accuracy, although does better on train loss. Finally, approaches like one cycle learning~(\cite{smith2018disciplined_onecycle,walk-with-sgd-2018}) have been proposed that linearly increase and decrease the learning rate in a specific manner. Based on our evaluation, one cycle scheme works reasonably well with manual tuning of the learning rate but does not always achieve state-of-the-art accuracy.

==> sections/seed_sensitivity.tex <==
\section{Seed Sensitivity}
\label{sec:seed_sensitivity}

We performed a sensitivity analysis on the importance of the choice of seed learning rate for \system{}. We ran \system{} for Cifar-10 on Resnet-18 with different seeds in a 10x range. Table~\ref{tab:seed_senstivity_cifar} shows the average test accuracies over 3 runs for the different seeds. As shown, the seed learning rate can impact the final accuracy, but \system{} is not highly sensitive to it, especially in the lower ranges.

\begin{table}[h]
\small
\centering
\begin{tabular}{|c|c|}
  \hline
  Seed LR & Test Accuracy \\ \hline
  0.05  & 94.60 \\ \hline
  0.075  & 94.71 \\ \hline
  0.1   & 94.79 \\ \hline
  0.125 & 94.58 \\ \hline
  0.15  & 94.25 \\ \hline
\end{tabular}
\caption{Cifar-10 on Resnet-18 trained for 200 epochs with Momentum. We report averages over 3 runs.}
\label{tab:seed_senstivity_cifar}
\end{table}

==> sections/stochasticity.tex <==
\section{Handling Stochasticity}
\label{sec:stochasticity}

For computation of the quadratic coefficients in equation~\ref{eq:epsilon_quadratic_form}, we need to compute the loss values $\hat{L}(\epsilon)$ at multiple values of $\epsilon$. Note that in a typical DNN setting we never compute the full loss, but only a stochastic loss based on a given minibatch. This loss, however, can be noisy and throw off our estimate of $\epsilon_{min}$. To handle this we follow two simple strategies. The first is to use a bigger minibatch (called {\it superbatch}) for computing the loss values, and the second is to use the {\it same} superbatch for computing all the losses for a particular estimate. The same strategy is used when computing loss drop rates for the saturation threshold check. We use an integer multiple of minibatches to make a superbatch. This allows us to compute the superbatch loss by simply averaging multiple single batch forward passes,  and does not increase the peak GPU memory usage. We use a conservative superbatch size of 100 for all our examples. See section~\ref{sec:superbatch_size_selection} for details on selection of superbatch size.

Finally, as a safeguard we also added a {\it rollback} policy. In case our system makes a bad call on the learning rate change (most likely because of a bad superbatch sample), which leads to a reduction in loss drop rate, we rollback the decision and revert the state of the network to the time we made the learning rate change. Although, {\it rollback} triggers rarely, it is helpful in preventing the optimization from going astray because of one bad decision.
